The NLO multileg working group: summary report

This report summarizes the activities of the NLM working group of the Workshop "Physics at TeV Colliders", Les Houches, France, 11-29 June, 2007.

==> contributions <==
======================================================================
Introduction

======================================================================
Part I: New approaches
----------------------------------------------------------------------

\section{Four-dimensional unitarity cuts\protect\footnote{Contributing authors: R. Britto, P. Mastrolia}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\title{Comments on Unitarity Based One-loop Algorithms}

\author{R.~K.~Ellis$^1$, W.~T.~Giele$^2$, Z..~Kunszt$^3$}
\institute{
$^1$Fermilab, Batavia, IL 60510, USA\\
$^2$ETH, Zurich, Switzerland\\
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\title{Physical applications of the OPP method to compute
one-loop amplitudes}

\author{Giovanni Ossola$^{(1)}$ ,
 Costas G.~Papadopoulos$^{(1)}$ ,
 Roberto Pittau$^{(2,3)}$ }
\institute{
$^1$Institute of Nuclear Physics, NCSR Demokritos,
15310 Athens, Greece \\
$^2$Departamento de F\'{i}sica Te\'orica y del Cosmos,
Centro Andaluz de F\'{i}sica de Part\'{i}culas Elementales (CAFPE),
Universidad de Granada, E-18071 Granada, Spain \\
$^3$Dipartimento di Fisica Teorica, Universit\` a di Torino,
and INFN sezione di Torino, via P. Giuria 1, Torino, Italy}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\title{On-shell recursion relations}

\author{Ch. Schwinn$^1$, S. Weinzierl$^2$}
\institute{$^1$Institut f\"ur Theoretische Physik E, RWTH Aachen,
D - 52056 Aachen, Germany
\\$^2$Institut f{\"u}r Physik, Universit{\"a}t Mainz,
D - 55099 Mainz, Germany}


======================================================================
Part II: Improvements on standard techniques 
----------------------------------------------------------------------

\title{GOLEM: a semi-numerical approach to one-loop amplitudes}

\author{C.~Bernicot$^1$, T.~Binoth$^2$, J.-Ph.~Guillet$^1$, G.~Heinrich$^3$,
E.~Pilon$^1$, T.~Reiter$^2$}
\institute{$^1$LAPTH, CNRS and Universit\'e de Savoie, B.P. 110,
Annecy-le-Vieux 74951, France
\\
$^2$The University of Edinburgh, J.C.M.B., The King's Buildings,
Edinburgh EH9 3JZ, Scotland\\
$^3$IPPP, Department of Physics,
University of Durham, South Road,
Durham DH1 3LE, UK}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\title{Issues with the Landau singularities}
\author{C.~Bernicot, F~Boudjema, J.P.~Guillet, N.D.~Le and E.~Pilon}
\institute{LAPTH, CNRS-Universit\'e de Savoie, UMR 5108, 74941
Annecy-le-Vieux}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\title{Tensor one-loop integrals in exceptional phase-space regions}

\author{A.~Denner$^1$ and S.~Dittmaier$^{2}$}

\institute{
$^1$Paul Scherrer Institut, W\"urenlingen und Villigen, CH-5232 Villigen PSI, Switzerland\\
$^2$Max-Planck-Institut f\"ur Physik (Werner-Heisenberg-Institut), D-80805 M\"unchen, Germany
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\title{
Singularities in one-loop amplitudes from point of view of Reduction Method}

\author{G. Duplan\v ci\' c}
\institute{
Theoretical Physics Division,
Rudjer Boskovic Institute,
P. O. Box 180,
HR-10002 Zagreb,
Croatia
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

======================================================================
Part III: Cross sections
----------------------------------------------------------------------

\title{Tuned comparison of QCD corrections to $pp\to WW{+}jet{+}X$ at the LHC}

\author{T.~Binoth$^{1}$, J.~Campbell$^{2}$, S.~Dittmaier$^{3}$,
R.~K.~Ellis$^{4}$, S.~Kallweit$^{3}$, S.~Karg$^{5}$, N.~Kauer$^{6}$, G.~Sanguinetti$^{7}$,
P.~Uwer$^{8}$ and G.~Zanderighi$^{9}$}

\institute{
$^1$School of Physics, The University of Edinburgh, Edinburgh EH9 3JZ, UK \\
$^2$The University of Glasgow, Glasgow, UK  \\
$^3$Max-Planck-Institut f\"ur Physik (Werner-Heisenberg-Institut), D-80805 M\"unchen, Germany\\
$^4$Fermilab, Batavia, IL 60510, USA\\
$^5$Institute for Theoretical Physics E, RWTH Aachen, D-52056 Aachen, Germany \\
$^6$Institute for Theoretical Physics, University of W\"urzburg, D-97074 W\"urzburg, Germany \\
$^7$LAPTH, 9, Chemin de Bellevue BP 110, 74941 Annecy le Vieux, France \\
$^8$ ... \\
$^9$ Dept. of Theoretical Physics, University of Oxford, UK.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\title{
From the high energy limit of massive QCD amplitudes to the full mass
dependence}

\author{M. Czakon$^{1,2}$}
\institute{$^1$Institut f\"ur Theoretische Physik
  und Astrophysik, Universit\"at W\"urzburg,
  Am Hubland, D-97074 W\"urzburg, Germany
  \\$^2$Institute of Physics, University of Silesia,
  Uniwersytecka 4, PL-40007 Katowice, Poland}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\title{
Measurements of hard processes at the LHC}

\author{G. Dissertori}
\institute{Institute for Particle Physics, ETH Zurich,
8093 Zurich, Switzerland}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\title{
NNLO predictions for hadronic event shapes in  $e^+e^-$ annihilations}

\author{G.\ Dissertori$^1$,A.~Gehrmann--De Ridder$^2$,T.~Gehrmann$^3$,
E.W.N.~Glover$^4$,G.~Heinrich$^4$,H.~Stenzel$^5$}
\institute{$^1$ Institute for Particle Physics, ETH Zurich,
      8093 Zurich, Switzerland\\
$^2$ Institute for Theoretical Physics, ETH Zurich,
      8093 Zurich, Switzerland\\
$^3$ Institut f\"ur Theoretische Physik, Universit\"at Z\"urich,
8057 Z\"urich, Switzerland\\
$^4$ Institute of Particle Physics Phenomenology,
        University of Durham, Durham, DH1 3LE, UK\\
$^5$ II. Physikalisches Institut, Justus-Liebig Universit\"at Giessen,
D-35392 Giessen, Germany\\
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\title{Much can be said about massive amplitudes just from knowing their massless limit}

\author{A. Mitov$^{1,2}$ and S. Moch$^2$}
\institute{ $^1$ Department of Mathematical Sciences, University of
Liverpool, Liverpool L69 3BX, United Kingdom
\\$^2$Deutsches Elektronensynchrotron DESY,
Platanenallee 6, D--15738 Zeuthen, Germany}


======================================================================
Part IV: Parton showers 
----------------------------------------------------------------------

\title{Time-like Showers Based on Dipole-Antenna Radiation Functions}

\author{R.~Frederix$^1$, W.~T.~Giele$^2$, D.~A.~Kosower$^3$,
  P.~Z.~Skands$^{4,2}$} 
\institute{
$^1$CP3, Universit\'e catholique de Louvain, 2 Chemin du Cyclotron,
  B-1348 Louvain-la-Neuve, Belgium\\  
$^2$Theoretical Physics, Fermilab MS106, Box 500, Batavia, IL--60510, USA\\
$^3$Service de Physique Th\'eorique, 
 CEA--Saclay, F--91191 Gif-sur-Yvette cedex, France\\
$^4$CERN PH-TH, CH-1211 Geneva 23, Switzerland
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\title{
LLL subtraction and PS kinematics}

\author{S. Odaka}
\institute{High Energy Accelerator Research Organization (KEK),
1-1 Oho, Tsukuba, Ibaraki 305-0801, Japan}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\title{
A Parton-shower model based on Catani--Seymour dipole factorisation}

\author{S.~Schumann$^1$, F.~Krauss$^2$}
\institute{$^1$School of Physics, The University of Edinburgh, Edinburgh EH9 3JZ, UK
\\$^2$ Institute for Particle Physics Phenomenology, Durham University, Durham DH1 3LE, UK}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\title{Developments in leading order parton showers}

\author{D.~E.~Soper$^1$ and P.~Z.~Skands$^2$}
\institute{
$^1$University of Oregon, Eugene, Oregon 97403 USA
and CERN, Geneva, Switzerland\\
$^2$CERN PH-TH, Geneva 23, CH-1211, Switzerland (on leave from Fermilab)
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> makebib <==
#!/bin/sh
#########################################################################
# create bib file nlm07.bib from all other .bib files 
#########################################################################
rm -f nlm07.bib
for file in `ls -R | grep "\.bib"`
    do 
    echo $file
    echo "%%% references taken from file "$file"%%%" >> nlm07.bib
    rm `find . -name $file -print` 
    done

